OpenBA: An Open-sourced 15B Bilingual Asymmetric seq2seq Model Pre-trained from Scratch

Large language models (LLMs) with billions of parameters have demonstrated outstanding performance on various natural language processing tasks. This report presents OpenBA, an open-sourced 15B bilingual asymmetric seq2seq model, to contribute an LLM variant to the Chinese-oriented open-source model community. We enhance OpenBA with effective and efficient techniques as well as adopt a three-stage training strategy to train the model from scratch. Our solution can also achieve very competitive performance with only 380B tokens, which is better than LLaMA-70B on the BELEBELE benchmark, BLOOM-176B on the MMLU benchmark, GLM-130B on the C-Eval (hard) benchmark. This report provides the main details to pre-train an analogous model, including pre-training data processing, Bilingual Flan data collection, the empirical observations that inspire our model architecture design, training objectives of different stages, and other enhancement techniques. Additionally, we also provide the fine-tuning details of OpenBA on four downstream tasks. We have refactored our code to follow the design principles of the Huggingface Transformers Library, making it more convenient for developers to use, and released checkpoints of different training stages at https://huggingface.co/openBA. More details of our project are available at https://github.com/OpenNLG/openBA.git.

==> Data_Preparation.tex <==
\section{Dataset Collection}
\label{sec:dataset_collection}
This section presents the data collection and filtering process for each training stage: pre-training data for stage \uppercase\expandafter{\romannumeral1} and \uppercase\expandafter{\romannumeral2}~(Sec.~\ref{subsec:pretrain_data_filtering}), and Bilingual FLAN~(BiFLAN) data for stage \uppercase\expandafter{\romannumeral3}~(Sec.~\ref{subsec:bilingual_flan_data_collection}).

\subsection{Pre-training Data Collection and Filtering}
\label{subsec:pretrain_data_filtering}
During the per-training stage for OpenBT5, we follow the methods in previous work~\cite{touvron2023llama, zeng2022glm}, constructing a 400B bilingual wide-variety pre-training data corpus with a balanced combination of Chinese and English. Specifically, the corpus comprises 190B Chinese tokens, 190B English tokens, and 20B code tokens. For the English portion, we sample from the Pile~\cite{gao2020pile} corpus, which is constructed from 22 diverse high-quality subsets. In particular, the code part of the data set is also sampled from the Pile, ensuring that the total code ratio is similar to that of LLaMA~\cite{touvron2023llama}. For the Chinese portion, we primarily sourced from the Internet and integrated datasets from books, encyclopedias, laws, reviews, news, and forums. Fig.~\ref{fig:pretrain_collection} shows the composition of the pre-training dataset. In both the UL2 pre-training stage, which utilizes 178B tokens, and the length-adaptation stage, which utilizes 42B tokens, we ensure there is no duplicate data.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figure/data_collection/pretrain_data_chart.pdf}
%     \caption{The composition of Pre-training Data Collection.}
%     \label{fig:pretrain_data}
% \end{figure}

\begin{figure}[t]
\centering
\subfigure[]{\includegraphics[width=0.32\linewidth]{figure/data_collection/pretrain_chart_new.pdf}\label{fig:pretrain_collection}}
\hfill
\subfigure[]{\includegraphics[width=0.32\linewidth]{figure/data_collection/biflan_chart_new.pdf}\label{fig:biflan_collection}}
\hfill
\subfigure[]{\includegraphics[width=0.32\linewidth]{figure/data_collection/zh_chart_new.pdf}\label{fig:cflan_collection}}
\caption{The composition of Data collection. Figure (a) represents the composition ratio of the pre-training dataset. Figure (b) represents the composition of the bilingual Flan dataset. Figure (c) represents the finer-grained composition of the Chinese Flan dataset.}
\label{fig:data_collection}
\end{figure}

% \subfigure[]{}
% \begin{figure}
%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

When constructing the pre-training dataset, we designed the filtering strategy based on previous works~\cite{sun2021ernie}, considering both personal privacy protection and data quality improvement:
\begin{itemize}
    \item Privacy Filter: To prevent potential privacy breaches, we removed all phone numbers, email addresses, and web links from the corpus.
    \item Deduplicate: At the character level, redundant characters are deleted, and sequences of repeated characters are trimmed to a single instance. At the paragraph level, we use a hash algorithm and sentence segmenter to identify and remove repeated sentences or paragraphs(we treat consecutive 1-99 sentences as a paragraph), retaining only unique versions. At the document level, we review all data sources to ensure there's no duplicate content across different datasets.
    \item Language Filter: We use polyglot\footnote{\url{https://github.com/aboSamoor/polyglot}} to detect the language of the text and only keep the texts with high confidence in either Chinese or English. We find it is useful to filter out gibberish, especially for texts extracted from PDFs via OCR algorithms.
    \item Internet Data Cleaning: Data collected from the Internet often suffers from incompletions, unrecognizable characters, and web page tags. Thus, we filter out sentences with less than 10 words and remove unusual characters and HTML tags.
    
\end{itemize}

\subsection{Bilingual Flan Data Collection}
\label{subsec:bilingual_flan_data_collection}
\paragraph{English Flan Data Collection}
The Flan Collection~\cite{chung2022scaling, longpre2023flan} serves as a foundational dataset for effective instruction tuning, encompassing more than 1800 tasks. Given that the English Flan Collection is easy to obtain~\footnote{\url{https://github.com/google-research/FLAN/tree/main/flan/v2}}, our focus in this section will predominantly center on the methodology employed in the Chinese Flan Data Collection.


\paragraph{Chinese Flan Data Collection}
The pre-training phase is for LLMs to learn language understanding and generation capabilities, and the instruction tuning stage is significant for LLMs to learn the ability of instruction-following which is able to understand all kinds of natural language prompts and generate satisfactory responses. Alpaca~\cite{alpaca} has proved that high-quality and diverse demonstrations are crucial for good instruction-following performance. 
However, most open-source instruction datasets are directly translated from English instruction datasets to Chinese~\cite{Luotuo} or generated by ChatGPT~\cite{ouyang2022training,bubeck2023sparks} by providing it with various prompts. The above methods respectively may exit the issues of translation errors and inaccurate answers. In a word, the current open-source Chinese instruction corpora are either of questionable quality or have a small amount. Therefore, inspired to alleviate the above problems, we develop our own Chinese instruction corpora. The details of collecting are as follows.

We collect 18 types of datasets, including 145 tasks and about 70 million pieces of data. All the datasets are collected from Natural Language Processing Competitions, Papers and open source high-quality datasets which could be found on the Web. The details of each task and data source could be found in Appendix A. For each dataset, we manually write a script to process it into a unified format and use natural language to construct instruction-prompt templates, ensuring the texts of the instruction prompt are concise and correct.
In our instruction-tuning stage, we actually use 5 million pieces of Chinese instruction datasets while merging part of the English Flan Collection. As shown in Figure~\ref{fig:biflan_collection}, the bilingual Flan dataset is composed of 66.7\% English Flan and 33.3\% Chinese Flan, and Figure~\ref{fig:cflan_collection} shows the composition of our Chinese Flan dataset in instruction-tuning stage, including 44 tasks within 18 types.


% 2.1 Collect from games (NLPCC、CCKS，CCL、paper with code、kaggle、TianChi), open source datasets (qianyan)





==> table/RACE.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{l c c c c}
    \toprule
    \bf Model & \bf \#Param. & \bf RACE-middle & \bf RACE-high \\
    \midrule
    GPT3 & 175B & 58.4 & 45.5 \\
    \midrule
    \multirow{3}{*}{PaLM} & 8B & 57.9 & 42.3 \\
                          & 62B & 64.3 & 47.5 \\
                          & 540B & 68.1 & 49.1 \\
    \midrule
    \multirow{4}{*}{LLaMA} & 7B & 61.1 & 46.9\\
                           & 13B & 61.6 & 47.2 \\
                           & 33B & 64.1 & 48.3 \\
                           & 65B & 67.9 & 51.6 \\
    \midrule
    OpenBA & 15B & 78.0 & 67.1 \\
    \bottomrule
    \end{tabular}
    \caption{Model performance on RACE benchmark, Zero-shot accuracy}
    \label{tab:race_results}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \begin{tabular}{|c|c|}
%             \hline
%             Column1 & Column2 \\
%             \hline
%             A & B \\
%             C & D \\
%             \hline
%         \end{tabular}
%         \caption{First table}
%         \label{tab:table1}
%     \end{minipage}\hfill
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \begin{tabular}{|c|c|}
%             \hline
%             Column1 & Column2 \\
%             \hline
%             E & F \\
%             G & H \\
%             \hline
%         \end{tabular}
%         \caption{Second table}
%         \label{tab:table2}
%     \end{minipage}
% \end{table}







==> table/chinese_data.tex <==
\begin{table}[th]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c}
    \toprule
    \bf Domain & \bf Ratio \\
    \midrule
    Internet & 60.3\% \\
    Books & 25.8\% \\
    Forums & 11.5\% \\
    News & 1.1\% \\
    Encyclopedias & 0.7\% \\
    Laws & 0.3\% \\
    Reviews & 0.3\% \\
    \bottomrule
    \end{tabular}
    \caption{The composition of the Chinese data collection.}
    \label{tab:chinese_data}
\end{table}

==> table/eval_template.tex <==
\begin{table}[th]
    \centering
    \small
    \begin{tabular}{ll}
    \toprule
    \bf Task   & \bf Template for instruction / zero-shot / chain-of-thought \\
    \midrule
         &  \\
    \bottomrule
    \end{tabular}
    \caption{Template for evaluation}
    \label{tab:template_for_evaluation}
\end{table}

==> table/machine_translation.tex <==
\begin{table}[t]
    \small
    \centering
    \begin{tabular}{l c c c}
        \toprule
        \bf Model & \bf \#Param. & \textbf{Zh}$\Rightarrow$\textbf{En} & \textbf{En}$\Rightarrow$\textbf{Zh} \\
        \midrule
        ChatGLM & 6B & 17.2 & \underline{32.5} \\
        Alpaca & 7B & 15.1 & 9.8 \\
        Alpaca-LoRA & 7B & 16.4 & 14.5 \\
        PARROT & 7B & \underline{19.6} & 24.8 \\
        BatGPT & 15B & \underline{23.1} & \bf 38.7 \\
        MOSS & 16B & 17.2 & 32.5 \\
        \midrule
        OpenBA & 15B & \textbf{23.3} & \underline{37.4} \\
        \bottomrule
    \end{tabular}
    \caption{Model performance on Flores subset containing 50 sentences sampled from Flores benchmark, where \#Param. denotes the model parameters. We report BLEU for all the models}
    \label{tab:mt_results}
\end{table}
    

==> table/mt.tex <==
% \begin{table}[ht]
%     \centering
%     \small
%     \begin{tabular}{l c c c}
%     \toprule
%     Model & \#Param. & \textbf{Zh}$\Rightarrow$\textbf{En} & \textbf{En}$\Rightarrow$\textbf{Zh} \\
%     \midrule
%     LLaMA & 7B & 1.86 & 0.05 \\
%     Alpaca & 7B & 15.13 & 9.81 \\
%     Alpaca-LoRA & 7B & 16.42 & 14.51 \\
%     MOSS & 16B & 17.2 & 32.5 \\
%     BatGPT & 15B & 23.1 & 38.7 \\
%     ChatGLM & 6B & 17.2 & 32.5 \\
%     \midrule
%     OpenBA & 14B & 23.0 & 37.5 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Model performance on Flores subset containing 50 sentences sampled from Flores benchmark, where \#Param. denotes the model parameters. We report BLEU for all baselines}
%     \label{tab:mt_results}
% \end{table}

==> table/roc.tex <==
\begin{table}[t]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c c c c c}
    \toprule
    \bf Model & \bf \#Param. & \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$)& \\
    \midrule
    BatGPT & 15B & 4.5 & 0.4 & \textbf{97.2} & 46.1 & \textbf{16.5} \\
    chatGLM & 6B & 5.0 & 0.3 & 99.9 & 5.35 & 14.8 \\
    MOSS & 16B & \textbf{5.8} & 0.3 & 99.7 & 37.34 & 14.8 \\
    OpenBA & 15B & \textbf{5.8} & \textbf{0.6} & 99.0 & \textbf{74.63} & 14.5 \\
    \bottomrule
    \end{tabular}
    \caption{Model performance on ROC, where \#Param. denotes the model parameters}
    \label{tab:roc}
\end{table}

% \begin{table}[t]
%     \centering
%     \small
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l c c c c c c | c c c c c}
%     \toprule
%     \multirow{2}{*}{\bf Model} & \bf \multirow{2}{*}{\#Param.} & \multicolumn{5}{c|}{\bf QQP} & \multicolumn{5}{c}{\bf WIKI AUTO}\\
%     \cmidrule{3-12}
%     & & \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$)& \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$)  \\
%     \midrule
%     BatGPT & 15B & 25.5 & 1.51 & 89.9 & 96.45 & 5.51 & 19.44 & 1.57 & 67.6 & 58.3 & 7.64 \\
%     chatGLM & 6B & 29.16 & 1.41 & 90.7 & 97.66 & 4.04 & 25.03 & 1.96 & 63.9 & 93.58 & 5.64 \\
%     MOSS & 16B & 27.83 & 1.49 & 82.9 & 96.8 & 5.42 & 19.31 & 1.36 & 72.7 & 37.18 & \textbf{7.78} \\
%     OpenBA & 15B & \textbf{32.67} & \textbf{1.74} & \textbf{77.1} & \textbf{98.8} & \textbf{5.58} & \textbf{27.69} & \textbf{2.1} & \textbf{46.8} & \textbf{94.97} & 6.62 \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Model performance on WIKU AUTO and QQP datasets.}
%     \label{tab:wiki_qqp}
% \end{table}

% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{l c c c c c c | c c c c c}
%     \toprule
%     \multirow{2}{*}{\bf Model} & \bf \multirow{2}{*}{\#Param.} & \multicolumn{5}{c}{\bf WIKI AUTO} \\
%     \cmidrule{3-7}
%     & & \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$) \\
%     \midrule
%     BatGPT & 15B & 25.5 & 1.51 & 89.9 & 96.45 & 5.51 \\
%     chatGLM & 6B & 29.16 & 1.41 & 90.7 & 97.66 & 4.04 \\
%     MOSS & 16B & 27.83 & 1.49 & 82.9 & 96.8 & 5.42 \\
%     OpenBA & 15B & \textbf{32.67} & \textbf{1.74} & \textbf{77.1} & \textbf{98.8} & \textbf{5.58} \\
%     \midrule
%     \multirow{2}{*}{\bf Model} & \bf \multirow{2}{*}{\#Param.} & \multicolumn{5}{c}{\bf ROC} \\
%     % & & \multicolumn{5}{c|}{\bf QQP} & \multicolumn{5}{c}{\bf WIKI AUTO}\\
%     \cmidrule{3-7}
%     & & \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$) \\
%     \midrule
%     BatGPT & 15B & 4.54 & 0.37 & \textbf{97.2} & \textbf{46.05} & \textbf{16.47} \\
%     chatGLM & 6B & 5.02 & 0.33 & 99.9 & 5.35 & 14.76 \\
%     MOSS & 16B & 5.76 & 0.33 & 99.7 & 37.34 & 14.84 \\
%     OpenBA & 15B & \textbf{6.0} & \textbf{0.63} & 99.5 & 29.88 & 13.78 \\
%     \midrule
%     \multirow{2}{*}{\bf Model} & \bf \multirow{2}{*}{\#Param.} & \multicolumn{5}{c}{\bf QQP} \\
%     % & & \multicolumn{5}{c|}{\bf QQP} & \multicolumn{5}{c}{\bf WIKI AUTO}\\
%     \cmidrule{3-7}
%     & & \bf B-2~($\uparrow$) & \bf D-2~($\uparrow$) & \bf LR-2~($\downarrow$) & \bf Mav~($\uparrow$) & \bf SIM~($\uparrow$) \\
%     \midrule
%     BatGPT & 15B & 19.44 & 1.57 & 67.6 & 58.3 & 7.64 \\
%     chatGLM & 6B & 25.03 & 1.96 & 63.9 & 93.58 & 5.64 \\
%     MOSS & 16B & 19.31 & 1.36 & 72.7 & 37.18 & \textbf{7.78} \\
%     OpenBA & 15B & \textbf{27.69} & \textbf{2.1} & \textbf{46.8} & \textbf{94.97} & 6.62 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Model performance on WIKU AUTO, ROC and QQP, where \#Param. denotes the model parameters}
%     \label{tab:story_generation}
% \end{table}


==> table/zero_clue.tex <==
\paragraph{Zero-shot CLUE}
\begin{table}[th]
    \centering
    \small
    \begin{tabular}{l c c c c c c }
    \toprule
    \bf Model & \bf \#Param. & \bf EPRSTMT & \bf OCNLI-FC & \bf BUSTM  & \bf CHID-FC  & \bf CLUEWSC-FC \\
    \midrule
    ERNIE 3.0 & 220B & 88.8 & 53.8 & 64.4 & 87.1 & 53.5 \\
    GLM-130B  & 130B & 92.5 & 73.8 & 77.5 & 90.1 & 72.4 \\                    
    \midrule
    OpenBA   & 15B  & 93.8 & 75.0 & 81.2 & 64.3 & 90.6 \\
    \bottomrule
    \end{tabular}
    \caption{Model performance on ZEROCLUE benchmark, Zero-shot accuracy}
    \label{tab:race_results}
\end{table}
